Subscriptions and external links help drive resentful users to alternative and extremist YouTube videos

Do online platforms facilitate the consumption of potentially harmful content? Using paired behavioral and survey data provided by participants recruited from a representative sample in 2020 (n=1,181), we show that exposure to alternative and extremist channel videos on YouTube is heavily concentrated among a small group of people with high prior levels of gender and racial resentment. These viewers often subscribe to these channels (prompting recommendations to their videos) and follow external links to them. In contrast, non-subscribers rarely see or follow recommendations to videos from these channels. Our findings suggest YouTube's algorithms were not sending people down "rabbit holes" during our observation window in 2020, possibly due to changes that the company made to its recommender system in 2019. However, the platform continues to play a key role in facilitating exposure to content from alternative and extremist channels among dedicated audiences.

==> tables/additional_regressions_hs_rr.tex <==

\begin{table}[!htbp]
  \caption{Correlates of time spent on YouTube videos by channel type \label{tab:additional-reg}} 
\fontsize{9}{10}\selectfont
\begin{center}
\begin{tabular}{@{\extracolsep{5pt}}lcccccc} 
\toprule
 & \multicolumn{6}{c}{\textit{Dependent variable: Time elapsed}} \\ 
\cline{2-7}
& \multicolumn{2}{c}{Alternative} & \multicolumn{2}{c}{Extremist} & \multicolumn{2}{c}{Mainstream} \\ 
& \multicolumn{2}{c}{channel videos} & \multicolumn{2}{c}{channel videos} & \multicolumn{2}{c}{channel videos} \\ 
& (1) & (2) & (3) & (4) & (5) & (6)\\ 
\midrule
Hostile sexism    & $1.95^{***}$ &              & $1.02$       &              & $-0.25$       &               \\
                  & $(0.53)$     &              & $(0.64)$     &              & $(0.30)$      &               \\
Racial resentment &              & $1.60^{**}$  &              & $1.14$       &               & $-0.45$       \\
                  &              & $(0.50)$     &              & $(1.00)$     &               & $(0.43)$      \\
Feeling Jews      & $-0.01$      & $-0.01$      & $-0.01$      & $-0.01$      & $0.01$        & $0.01$        \\
                  & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.01)$     & $(0.02)$      & $(0.02)$      \\
Democrat          & $-1.98^{**}$ & $-1.66^{**}$ & $-2.46^{*}$  & $-2.15$      & $0.40$        & $0.04$        \\
                  & $(0.74)$     & $(0.60)$     & $(1.09)$     & $(1.17)$     & $(0.81)$      & $(1.03)$      \\
Republican        & $-2.26^{*}$  & $-2.28^{**}$ & $-0.50$      & $-0.70$      & $-0.13$       & $0.09$        \\
                  & $(1.02)$     & $(0.81)$     & $(1.32)$     & $(1.32)$     & $(0.82)$      & $(0.70)$      \\
Age               & $0.04$       & $0.00$       & $0.03$       & $0.02$       & $0.04^{**}$   & $0.04^{**}$   \\
                  & $(0.03)$     & $(0.02)$     & $(0.02)$     & $(0.02)$     & $(0.01)$      & $(0.01)$      \\
Male              & $0.56$       & $1.15$       & $0.28$       & $0.56$       & $0.94$        & $0.95$        \\
                  & $(1.08)$     & $(0.84)$     & $(1.29)$     & $(0.91)$     & $(0.64)$      & $(0.68)$      \\
Non-white         & $-0.54$      & $-0.85$      & $-0.92$      & $-1.06$      & $1.41$        & $1.45$        \\
                  & $(0.92)$     & $(1.05)$     & $(0.92)$     & $(0.99)$     & $(0.84)$      & $(0.85)$      \\
Some college      & $0.45$       & $0.70$       & $0.25$       & $0.40$       & $1.42^{*}$    & $1.48^{*}$    \\
                  & $(1.03)$     & $(0.86)$     & $(0.88)$     & $(0.83)$     & $(0.69)$      & $(0.70)$      \\
Bachelor's degree & $1.60$       & $1.26$       & $0.75$       & $0.74$       & $2.45^{***}$  & $2.45^{***}$  \\
                  & $(1.18)$     & $(1.09)$     & $(1.05)$     & $(0.98)$     & $(0.69)$      & $(0.72)$      \\
Post-grad         & $-0.47$      & $-0.51$      & $-1.84^{*}$  & $-1.80^{*}$  & $2.68^{***}$  & $2.62^{***}$  \\
                  & $(1.01)$     & $(1.11)$     & $(0.92)$     & $(0.81)$     & $(0.69)$      & $(0.69)$      \\
Intercept         & $-3.45$      & $-0.20$      & $-1.59$      & $-1.61$      & $0.39$        & $0.91$        \\
                  & $(3.69)$     & $(2.37)$     & $(2.05)$     & $(2.47)$     & $(2.60)$      & $(2.52)$      \\
\midrule
N         & $847$        & $847$        & $847$        & $847$        & $847$         & $847$         \\
\bottomrule
\multicolumn{7}{l}{\scriptsize{$^{***}p<0.001$; $^{**}p<0.01$; $^{*}p<0.05$}}
\end{tabular}
\end{center}
\footnotesize{Quasipoisson coefficients for correlates of time per week spent on videos from alternative, extremist, and mainstream media channels. Robust standard errors are in parentheses.}
\end{table}


==> tables/external_referrers_by_channel_type.tex <==
\begin{table}[!htbp]
\caption{\label{tab:externalrefs}External referrers to alternative and extremist channel videos}
\centering
\begin{tabular}[t]{llrr}%
\toprule
Referrer type & Preceding domain & \% extremist channel & \% alternative channel\\
& & external referrers & external referrers \\
\midrule
Alternative social & 4chan.org & 0.09 & 0.00\\
 & banned.video & 0.00 & 0.05\\
 & boards.4chan.org & 0.58 & 0.35\\
& boards.4channel.org & 0.94 & 0.41\\
 & gab.com & 1.21 & 1.62\\
 & parler.com & 0.40 & 1.39\\
 & twitchy.com & 28.88 & 0.68\\
 \addlinespace
Mainstream social & apps.facebook.com & 0.40 & 0.25\\
 & bumble.com & 0.00 & 0.05\\
 & discord.com & 0.00 & 0.08\\
 & facebook.com & 8.59& 16.61\\
 & instagram.com & 0.04 & 0.54\\
 & linkedin.com & 0.13& 0.12\\
 & messenger.com & 1.12 & 2.05\\
 & old.reddit.com & 0.54 & 0.75\\
 & pinterest.com & 0.00 & 0.05\\
 & reddit.com & 0.72 & 1.67\\
 & tinder.com & 0.04 & 0.38\\
 & tumblr.com & 0.00 & 0.19\\
 & twitch.tv & 0.18 & 0.97\\
 & twitter.com & 8.59 & 7.65\\
 \addlinespace
Search engine & bing.com & 0.54 & 0.64\\
 & duckduckgo.com & 0.45 & 1.48\\
 & google.com & 5.26 & 4.86\\
 & search.yahoo.com & 0.09 & 0.14\\
 & yahoo.com & 0.27 & 0.27\\
  \addlinespace
Webmail & mail.aol.com & 0.18 & 0.26\\
 & mail.com & 0.00 & 0.03\\
& mail.google.com & 3.73 & 6.50\\
& mail.yahoo.com & 1.89 & 1.70\\

 & outlook.live.com & 0.13 & 0.56\\
 & outlook.office.com & 0.00 & 0.02\\
 & outlook.office365.com & 0.00 & 0.02\\
\bottomrule
\end{tabular}
\end{table}

